Efficient Explanations from Empirical Explainers

Amid a discussion about Green AI in which we see explainability neglected, we explore the possibility to efficiently approximate computationally expensive explainers. To this end, we propose feature attribution modelling with Empirical Explainers. Empirical Explainers learn from data to predict the attribution maps of expensive explainers. We train and test Empirical Explainers in the language domain and find that they model their expensive counterparts surprisingly well, at a fraction of the cost. They could thus mitigate the computational burden of neural explanations significantly, in applications that tolerate an approximation error.

==> acl2020.tex <==
%
% File acl2020.tex
%
%% Based on the style files for ACL 2020, which were
%% Based on the style files for ACL 2018, NAACL 2018/19, which were
%% Based on the style files for ACL-2015, with some improvements
%%  taken from the NAACL-2016 style
%% Based on the style files for ACL-2014, which were, in turn,
%% based on ACL-2013, ACL-2012, ACL-2011, ACL-2010, ACL-IJCNLP-2009,
%% EACL-2009, IJCNLP-2008...
%% Based on the style files for EACL 2006 by 
%%e.agirre@ehu.es or Sergi.Balari@uab.es
%% and that of ACL 08 by Joakim Nivre and Noah Smith




% \documentclass[11pt,a4paper]{article}
% \usepackage[hyperref]{acl2021}
% \usepackage{times}
% \usepackage{booktabs}
% \usepackage{array}
% \usepackage{latexsym}
% \usepackage{verbatim}
% \usepackage{arydshln}
% %\usepackage{subcaption}
% \usepackage{enumitem}
% \usepackage{pgfplots}
% \usepgfplotslibrary{units}
% \pgfplotsset{unit code/.code 2 args={\si{#1#2}}}
% \usetikzlibrary{patterns}
% \usepackage{siunitx}
% \usepackage{subfigure}
% \renewcommand{\UrlFont}{\ttfamily\small}

% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}
% \usepackage{xcolor}
% \usepackage{soul}
% \usepackage{enumitem}% http://ctan.org/pkg/enumitem
% %  plus4mm minus3mm}

% \usepackage{amsmath}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}


% \aclfinalcopy % Uncomment this line for the final submission
% %\def\aclpaperid{***} %  Enter the acl Paper ID here

% %\setlength\titlebox{5cm}
% % You can expand the titlebox if you need extra space
% % to show all the authors. Please do not make the titlebox
% % smaller than 5cm (the original size); we will check this
% % in the camera-ready version and ask you to change it back.

% \newcommand\BibTeX{B\textsc{ib}\TeX}

% \title{Efficient Explanations from Empirical Explainers}


% \author{Robert Schwarzenberg$^1$ \\ \And Nils Feldhus$^1$ \\ $^1$German Research Center for Artificial Intelligence (DFKI) \\ $^2$Technische Universität Berlin (TU Berlin) \\
%   \texttt{\{firstname.lastname\}@dfki.de} \And Sebastian Möller$^{1,2}$}
  
% %\usepackage[printwatermark]{xwatermark}
% %\newwatermark[allpages,color=red!30,angle=45,scale=3,xpos=0,ypos=0]{DRAFT\\ \small Do Not Distribute}

% \date{}

% \input{results-data/bert-imdb-ig}
% \input{results-data/xlnet-snli-svs}

% \begin{document}
% %\setlength{\abovedisplayskip}{3pt}
% %\setlength{\belowdisplayskip}{3pt}
% \raggedbottom


% \maketitle
% \input{sections/abstract}
% \input{sections/introduction}
% \input{sections/expensive-explainers}
% \input{sections/empirical-explainers}
% \input{sections/experiments}
% \input{sections/results}
% \input{sections/related-work}
% \input{sections/conclusion-future-work}
% \bibliography{anthology,acl2021, literature}
% \bibliographystyle{acl_natbib}
% %\input{sections/appendix}
% \end{document}

